Nonequilibrium Statistical Physics in Ecology: Vegetation Patterns, Animal Mobility and Temporal Fluctuations

This thesis focuses on the applications of mathematical tools and concepts brought from nonequilibrium statistical physics to the modeling of ecological problems. The first part provides a short introduction where the theoretical concepts and mathematical tools that are going to be used in subsequent chapters are presented. Firstly, the different levels of description usually employed in the models are explained. Secondly, the mathematical relationships among them are presented. Finally, the notation and terminology that will be used later on are explained. The second part is devoted to studying vegetation pattern formation in regions where precipitations are not frequent and resources for plant growth are scarce. This part comprises two chapters. The third part of the thesis develops a series of mathematical models describing the collective movement and behavior of some animal species. Its primary objective is to investigate the effect that communication among foragers has on searching times and the formation of groups. It consists of two chapters. The fourth part covers the effect of stochastic temporal disorder, mimicking climate and environmental variability, on systems formed by many interacting particles. These models may serve as an example of ecosystems. The thesis ends with a summary and devising future research lines.

==> pfc_dedicatoria.tex <==
%
% Dedicatoria
%
\chapter*{}
\begin{flushright}
	{\it aaaaaa.}
\end{flushright}

